Integrating Image Features with Convolutional Sequence-to-sequence Network for Multilingual Visual Question Answering

Visual Question Answering (VQA) is a task that requires computers to give correct answers for the input questions based on the images. This task can be solved by humans with ease but is a challenge for computers. The VLSP2022-EVJVQA shared task carries the Visual Question Answering task in the multilingual domain on a newly released dataset: UIT-EVJVQA, in which the questions and answers are written in three different languages: English, Vietnamese and Japanese. We approached the challenge as a sequence-to-sequence learning task, in which we integrated hints from pre-trained state-of-the-art VQA models and image features with Convolutional Sequence-to-Sequence network to generate the desired answers. Our results obtained up to 0.3442 by F1 score on the public test set, 0.4210 on the private test set, and placed 3rd in the competition.

==> sections/final_visualize.tex <==
\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/GoodCaseSeaShips/002109.jpg}
    \label{fig:badcase1} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/GoodCaseSeaShips/006637.jpg} 
    \label{fig:badcase2} 
    \vspace{4ex}
  \end{subfigure} 
  
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/GoodCaseSeaShips/005455.jpg}
    \label{fig:badcase3} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/GoodCaseSeaShips/006950.jpg}
    \label{fig:badcase4} 
  \end{subfigure}
  \label{fig7} 
  \caption{Some perfect cases of DLAFS Cascade R-CNN on SeaShips dataset}
  \label{fig:goodcases}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/BadCaseSeaShips/000654.jpg}
    \label{fig7:a} 
    \caption{SeaShip bad case 1}
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/BadCaseSeaShips/006410.jpg} 
    \label{fig7:b} 
    \caption{SeaShip bad case 2}
    \vspace{4ex}
  \end{subfigure} 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/BadCaseSeaShips/006500.jpg}
    \caption{SeaShip bad case 3}
    \label{fig7:c} 
  \end{subfigure}%%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/BadCaseSeaShips/002378.jpg}
    \caption{SeaShip bad case 2}
    \label{fig7:d} 
  \end{subfigure}
  \label{fig7} 
  \caption{Some bad cases of DLAFS Cascade R-CNN on SeaShips dataset. Ignored objects and wrong objects are circled in red and white respectively.}
%   (a) Distant ships are unrecognizable; (c) A distant bulk cargo carrier is mistaken with the other shore; (d) Ships that are overlapped each other will be misrecognized
  \label{fig:badcases}
\end{figure}

\begin{figure}[H]
  \centering
  \begin{subfigure}[b]{0.55\linewidth}
    \centering
    \includegraphics[width=0.85\linewidth]{images/CascadeDODV/104.jpg}
    \label{fig:badcaseDODV1} 
    \vspace{4ex}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.55\linewidth}
    \centering
    \includegraphics[width=0.8\linewidth]{images/CascadeDODV/CTU_060400067.jpg}
    \label{fig:badcaseDODV2} 
    \vspace{4ex}
  \end{subfigure} 
\vspace{-1.3cm}
  \caption{Some perfect cases of DLAFS Cascade R-CNN on DODV dataset}
  \label{fig:goodcasesDODV}
  \vspace{-1.5cm}
\end{figure}



\begin{figure}[H]
	  \centering
  \begin{subfigure}[b]{0.55\linewidth}
    \centering
    \includegraphics[width=0.75\linewidth]{images/CascadeDODV/Tep_001.jpg}
    \label{fig:badcaseDODV1} 
    %\vspace{4ex}
    %\vspace{-.5cm}
    \caption{DODV bad case 1}
  \end{subfigure}%% 
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[width=.91\linewidth]{images/CascadeDODV/CTU_060400071.jpg}
    \label{fig:badcaseDODV2} 
    %\vspace{4ex}
    \vspace{-.5cm}
    \caption{DODV bad case 2}
  \end{subfigure} 
  \caption{Some bad cases of DLAFS Cascade R-CNN on DODV dataset. Wrong predictions are zoned in red color.}
  \label{fig:badcasesDODV}
\end{figure}

\begin{figure*}[H]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_1-1.pdf}
     \end{subfigure}
     \hspace{6mm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_2-2.pdf}
     \end{subfigure}
     \vspace{6mm}
     
     
     \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_3-3.pdf}
     \end{subfigure}
     \hspace{6mm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_4-4.pdf}
     \end{subfigure}
     \vspace{6mm}
     
     
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_5-5.pdf}
     \end{subfigure}
     \hspace{6mm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_6-6.pdf}
     \end{subfigure}
     \vspace{6mm}
     
     
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_7-7.pdf}
     \end{subfigure}
     \hspace{6mm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/MS-COCO/coco_example_8-end.pdf}
     \end{subfigure}
     \vspace{6mm}
     
     %chúng tôi trực quan một phần của ảnh
     \caption{Visualization results of DLAFS Cascade R-CNN on MS-COCO }
     \label{fig:ms-coco}
\end{figure*}
